IBM Federated Learning: an Enterprise Framework White Paper V0.1

Federated Learning (FL) is an approach to conduct machine learning without centralizing training data in a single place, for reasons of privacy, confidentiality or data volume. However, solving federated machine learning problems raises issues above and beyond those of centralized machine learning. These issues include setting up communication infrastructure between parties, coordinating the learning process, integrating party results, understanding the characteristics of the training data sets of different participating parties, handling data heterogeneity, and operating with the absence of a verification data set. IBM Federated Learning provides infrastructure and coordination for federated learning. Data scientists can design and run federated learning jobs based on existing, centralized machine learning models and can provide high-level instructions on how to run the federation. The framework applies to both Deep Neural Networks as well as ``traditional'' approaches for the most common machine learning libraries. {\proj} enables data scientists to expand their scope from centralized to federated machine learning, minimizing the learning curve at the outset while also providing the flexibility to deploy to different compute environments and design custom fusion algorithms.

==> arch.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\columnwidth]{ffl-3d.pdf}
    \caption{Three dimensions of {\proj}}
    \label{fig:ffl-3d}
\end{figure}

Setting up and deploying a federated learning system is not an easy task. It requires setting up a communication infrastructure, converting machine learning algorithms to federated settings and in some cases knowing about the intricacies of differential privacy and multi-party computation.


\textbf{The following only covers one of the users... (@Ali, I  introduced two types in the prior section.) We need to cover the developer too}

{\proj} allows data scientists and researchers to train a ML model in FL by specifying the model as they would normally do. The following simple steps can be followed: 

\paragraph{1. Define ML model} 
...
\paragraph{2. Specify Fusion algorithm to be used}
...
\paragraph{3. Specify FL configuration and list of parties}
...
\paragraph{4. Launch Aggregator and wait for quorum to start}
...


\subsection{Supported Functionalities} \textbf{Is this a wish list?}
{\proj} provides a platform that allows data scientist and researchers alike to speed up the process of developing and testing their federated learning system. With an architecture designed to allow to choose among different communication protocols independently of the machine learning tasks and a standard way to define machine learning models, {\proj} enables faster ways to train models without sharing data: 
\begin{itemize}
    \item Works with different ML frameworks (Keras, Scikit-learn, PyTorch)
    \item Runs learning parties and aggregators
    \item Enables fast definition of FL project, starting from centralized ML program
    \item Choose from framework libraries and algorithms
    \item Provides out of the box methods to train \emph{differential private} models to protect against data leakage 
    \item Enables \emph{multiple party computation} techniques to exchange model updates 
\end{itemize}

\paragraph{Machine Learning}
{\proj} supports various ML related functionalities. Table~\ref{table:ml} summarizes those features.

\begin{center}
\begin{table}
 \begin{tabular}{|c |c | c |} 
 \hline
 \textbf{ML Model} & \textbf{Fusion Algorithms} & \textbf{Model Wrappers} \\ [0.5ex] 
 \hline\hline
 Neural networks & Average aggregation  & Keras  \\ 
 \hline
 Decision Tree ID3 & Weighted aggregation & Scikit-learn  \\
 \hline
 Linear classifiers & PFNM aggregation & Tensorflow \\
 \hline
 Logistic regressions  & Decision Tree ID3 & Pytorch \\
 \hline
 XGBoost & Rubble band &  \\  
 \hline
 Naïve Bayes &&\\[1ex]
 \hline
\end{tabular}
\caption{Supported ML related functionalities}
\label{table:ml}
\end{table}
\end{center}

\paragraph{Connectivity}
For connectivity, {\proj} provides support for Flask, GRPC (ongoing), Publisher-Subscribe (ongoing), or TCP (plan) based connections. The flexibility in connectivity allows {\proj} to be used in a versatile range of FL applications, ranging from enterprise settings in cloud to IoT-like environments.

\paragraph{Privacy and Security}
For \epmh{Differential Privacy}, {\proj} supports  Neural networks, Naïve Bayes (ongoing), and Decision Tree (plan). For \emph{Secure Multi-party Computation}, {\proj} supports Additive homomorphic encryption (Paillier - ongoing)
Threshold additive homomorphic encryption (Threshold-Paillier - ongoing), and Functional encryption (ongoing).
\\

Additionally, new machine learning algorithms, cryptographic techniques and privacy enhancing techniques are constantly being designed. {\proj} is designed to enable adding new techniques and swapping underlying communication and infrastructure without the need to re-write all of the other components.

\subsection{Architecture}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\columnwidth]{ffl-arch.png}
    \caption{{\proj}'s architecture.}
    \label{fig:ffl-arch}
\end{figure}

{\proj} offers as abstraction an Aggregator and Parties (as shown in the figure below), so that a group of parties can collaboratively learn a machine learning model (usually referred to as a global model) without revealing their raw data to each other. For most of the existing federated learning algorithms, only model weights (aka model parameters/model updates) will be shared as either plain text or encrypted messages with the aggregator, and the aggregator can then learn a global model by aggregating the information provided by parties. We now introduce these two abstractions in {\proj}.

\paragraph{Aggregator} The aggregator is in charge of running the Fusion Algorithm. A fusion algorithm queries registered parties to carry out the federated learning process. The queries sent vary on the model/algorithm types utilized.  In return, parties send back their reply as a model update object, these model updates are then aggregated according to the specified Fusion Algorithm, specified via a Fusion Handler class.

\paragraph{Data party}
Each party holds its own data set that is kept to itself, and that is used to answer queries received from the aggregator. Because each party may have stored their data in different formats, {\proj} offers an abstraction called Data Handler. This module allows for custom implementations to retrieve the data from each of the participating parties. A local training handler sits at each party to control the local training happening at the party side.
\\

Additionally, the aggregator and parties can communicate through multiple communication mechanisms such as flask-based servers, pub-subscriber, and GPRC, among others. All messages and communication are handled by the protocol handler and connection modules.

\subsubsection{{\proj}'s Components}
{\proj} has built-in algorithms to train different kinds of machine learning models, e.g., neural networks, linear models and decision trees, in a federated learning fashion. Setting up a federated learning task in a real distributed environment is not an easy job.  To ease burdens like building a distributed system, handling protocols and managing message exchange, etc., {\proj} is designed to allow different modules to be swapped without interfering with the functionality of other components. Here are the components that can be selected for a learning project:

\begin{itemize}
    \item \textbf{Connection:} Connection types for communication between the aggregator and each registered party.
    \item \textbf{Data Handler:} Data preparation and preprocessing.
    \item \textbf{Fusion:} Fusion algorithm to be performed at the aggregator side.
    \item \textbf{Local Training:} Local training algorithm and prepare query responses at the party side.
    \item \textbf{Hyperparameters:} Global training and local training hyperparameters.
    \item \textbf{Model:} Definition of the machine learning model to be trained.
    \item \textbf{Protocol Handler:} Handling the protocol for message exchange.
\end{itemize}

\subsubsection{{\proj}'s functioning}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\columnwidth]{ffl-flow.pdf}
    \caption{{\proj}'s runtime flow.}
    \label{fig:ffl-flow}
\end{figure}


\subsubsection{Using {\proj}}


==> background.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{fl.pdf}
    \caption{Federated Learning Overview - Vanilla version}
    \label{fig:fl-overview}
\end{figure}

%\textit{\subsection{Federated Learning}}
In this section we dig into the intricacies of the federated learning training process, and explain the three different dimensions that underpin the design of our framework.

Figure~\ref{fig:fl-overview} shows a federated learning overview. Data Parties ($P_1$, $P_2$, $P_N$) each having their own data set ($D_1$, $D_2$, ..., $D_N$) and receive a Query ($Q$) from a central Aggregator to train a model locally. Once local training is completed, each party replies to the Aggregator with their trained model ($R_1$, $R_2$, ..., $R_N$). Once the Aggregator receives replies from all the parties, it fuses the received models together to generate one \emph{global model}. Then, this global model is shared with all the parties. This process is repeated either until a desired accuracy or a fixed number of (\emph{rounds}) is achieved.
We call the algorithm run by the Aggregator a \textit{fusion algorithm}.
% Example to make it concreete... 
As an example, when a neural network is being trained, the Aggregator may send an initial model and request new model weights, then each party uses this model to further fit it to the party's own data to train, and then returns its associated weights to the Aggregator. The Aggregator in turn averages the weights to find a new model and updates parties with it.


\textbf{I think we could skip this paragraph:}
Also, talk about types of FL from systems (central vs decentralized) and data perspective (Horizontal Vs. Vertical). Other types of ML concepts like transfer, unsupervised, etc.

There are multiple aspects that impact the algorithms and deployment of federated learning systems.




\subsection{Privacy and Security}
There is not a single \textit{fit-all} solution from the privacy and security perspective for the federated learning process.
As such, different privacy and security techniques need to be applied depending on the application where federated learning is run and the associated threat model.

The process described before (Figure \ref{fig:fl-overview}) provides privacy and satisfies some privacy legislation that simply required training data to remain local. For instance, a company that aims to train a machine learning model using data from its subsidiaries located in multiple geographical locations can simply apply this vanilla federated learning process.

However, for settings where participating parties do not trust each other or the aggregator, new factors need to be considered.
Although at first glance it may seem that this approach provides some level of privacy, attacks in the literature have demonstrated that it is possible to infer private information by inspecting the messages exchanged during the training process or querying the final or intermediate machine learning model produced
\cite{fredrikson2015model, shokri2017membership, nasr2019comprehensive}.

In order to mitigate these inference attacks,
it is necessary to incorporate additional provisions into the federated learning process.
Multiple techniques to deter these threats have been proposed to date.

\noindent \textbf{Multi-party computation} (MPC) is one such techniques, where parties 
 jointly compute a function over their model updates while keeping those inputs private. Adopting one such approach protects against attacks where individual replies are inspected to infer private data.
 The selection of the MPC cryptographic technique used ensures that a plethora of requirements are met, from preventing a curious aggregator \cite{homo}, to ensuring that even if other parties collude by manipulating their model updates \cite{threshold}, no private information can be inferred.

% DP 
\noindent \textbf{Differential privacy} has been considered as a way to protect against inference threats to the models produced as well as inference to the messages exchanged during the federated learning process.
Here, each participant uses a differential privacy mechanism to inject noise to the replies sent to the aggregator.
Because the reply is noisy, there is some mathematical guarantee that the risk of inference is limited. This can be seen as a plausible deniability of a reply.
It also protects against membership inference attacks to the final model \cite{x}. 
Unfortunately, it has been shown that applying un-coordinated differential private noise (local-DP) does not yield to good performing models unless a large number of parties are queried or transfer learning is in place \cite{ownership-inf-paper}.

% DP + MPC 
\noindent \textbf{Hybrid-approaches} have been proposed to achieve both privacy of the inputs and protect against membership inference attacks \cite{our-two-papers}. When coordinated DP-noise is added, model performance improves drastically. Hence, this is a good option for certain threat models. 
Given the dependency on the threat model and use case at hand, it would be very beneficial to have a framework that would allow to swap and switch different approaches during the training process. 

\subsection{Enterprise Setting Requirements}
Most of the work in the FL area has been tailored to mobile devices,
where data is stored in the same format in each device.
For enterprise-based federated learning, the situation is very different.
In fact, organizations often store their data in different formats and locations, going from data warehouses, to private and hybrid clouds.
In this setting, a framework that allows the transparent reconciliation of these formats and places where data is stored is needed.
Data pre-processing needs to be allowed as well.

\subsection{Deployment Requirements}
\textbf{Here talk about need for multiple connections pub-sub and so forth.}

\subsection{Developer and Data Scientist Requirements}
There are two types of users in federated learning: 
The developer of federated learning algorithms who wants to create and test new fusion algorithms and may want to modify the way parties train locally.
For the first type of user, it is desirable to enable a single point where they can specify the machine learning code and use high level APIs to query parties and retrieve replies.

A second type of user is a data scientist who wants to train, in federated learning fashion, a model specified in a well-known machine learning framework, such as Keras or Scikit. This type of user doesn't want to learn the intricacies of the fusion algorithms run in order to train and test multiple model types and hyperparameters. Similarly, they may select configurations such as desired privacy and security modules.





